Length Extrapolation of Transformers: A Survey from the Perspective of Positional Encoding

Built upon the Transformer, large language models (LLMs) have captured worldwide attention due to their remarkable abilities. Nevertheless, all Transformer-based models including LLMs suffer from a preset length limit and can hardly generalize from short training sequences to longer inference ones, namely, they cannot perform length extrapolation to handle long sequences, which severely hinders their application in scenarios demanding long input sequences such as legal or scientific documents. Thus, numerous methods have emerged to enhance the length extrapolation of Transformers. Despite the great research efforts, a systematic survey is still lacking. To fill this gap, we delve into these advances in a unified notation from the perspective of positional encoding (PE), as it has been considered the primary factor on length extrapolation. Specifically, we begin with extrapolatable PEs that have dominated this research field. Then, we dive into extrapolation methods based on them, covering position interpolation and randomized position methods. Finally, several challenges and future directions in this area are highlighted. Through this survey, we aim to enable the reader to gain a deep understanding of existing methods and provide stimuli for future research.

==> latex/category_tree_new.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
]
\tikzstyle{cause_leaf}=[my-box, minimum height=1.5em,
    fill=harvestgold!20, text=black, align=left,font=\scriptsize,
    inner xsep=2pt,
    inner ysep=4pt,
]
\tikzstyle{detect_leaf}=[my-box, minimum height=1.5em,
    fill=cyan!20, text=black, align=left,font=\scriptsize,
    inner xsep=2pt,
    inner ysep=4pt,
]
\tikzstyle{mitigate_leaf}=[my-box, minimum height=1.5em,
    fill=lightgreen!20, text=black, align=left,font=\scriptsize,
    inner xsep=2pt,
    inner ysep=4pt,
]
\begin{figure*}[tp]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\small,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=4.0em,font=\scriptsize,}{},
            where level=2{text width=7.5em,font=\scriptsize,}{},
            where level=3{text width=7.2em,font=\scriptsize,}{},
            where level=4{text width=6.4em,font=\scriptsize,}{},
            [
                Hallucinations in Large Language Models, ver, color=carminepink!100, fill=carminepink!15,
                text=black
                [
                    Hallucination \\ Causes (\S \ref{sec:causes}), color=harvestgold!100, fill=harvestgold!100, text=black
                    [
                        Hallucination from Data, color=harvestgold!100, fill=harvestgold!60,  text=black
                        [
                            Flawed Data Source, color=harvestgold!100, fill=harvestgold!40, text=black
                            	[
                            		Misinformation and \\ Biases, color=harvestgold!100, fill=harvestgold!20, text=black
                            		[
                                		{\eg~\citet{DBLP:conf/acl/LinHE22, lee2021deduplicating, bender2021dangers}}
                                		, cause_leaf, text width=20em
                            		]
                            ]
                            [
                            		Knowledge Boundary, color=harvestgold!100, fill=harvestgold!20, text=black
                            		[
                                		{\eg~\citet{singhal2023towards, katz2023gpt, onoe2022entity}}
                                		, cause_leaf, text width=20em
                            		]
                            ]  
                        ]
                        [
                            Inferior Data Utilization, color=harvestgold!100, fill=harvestgold!40, text=black
                            [
                            		Knowledge Shortcut, color=harvestgold!100, fill=harvestgold!20, text=black
                            		[
                                		{\eg~\citet{li2022pre, kandpal2023large, kang2023impact}}
                                		, cause_leaf, text width=20em
                            		]
                            ]  
                            [
                            		Knowledge Recall \\ Failures, color=harvestgold!100, fill=harvestgold!20, text=black
                            		[
                                		{\eg~\citet{DBLP:conf/acl/MallenAZDKH23, zheng2023does, DBLP:journals/corr/abs-2307-03172}}
                                		, cause_leaf, text width=20em
                            		]
                             ]  
                        ]
                    ]
                    [
                        Hallucination from \\ Training, color=harvestgold!100, fill=harvestgold!60, text=black
                        [
                            Hallucination from \\ Pre-training, color=harvestgold!100, fill=harvestgold!40, text=black
                            [
                            		Architecture Flaw, color=harvestgold!100, fill=harvestgold!20, text=black
                            		[
                                		{\eg~\citet{li2023batgpt, liu2023exposing}}
                                		, cause_leaf, text width=20em
                            		]
                            ]
                            [
                            		Suboptimal Training \\ Objective, color=harvestgold!100, fill=harvestgold!20, text=black
                            		[
                                		{\eg~\citet{wang2020exposure, zhang2023language}}
                                		, cause_leaf, text width=20em
                            		]
                            ]
                        ]
                        [
                            Hallucination from \\ Alignment, color=harvestgold!100, fill=harvestgold!40, text=black
                            [
                            		Capability \\ Misalignment, color=harvestgold!100, fill=harvestgold!20, text=black
                            		[
                                		{\eg~\citet{schulman2023youtube}}
                                		, cause_leaf, text width=20em
                            		]
                             ]
                             [
                            		Belief Misalignment, color=harvestgold!100, fill=harvestgold!20, text=black
                            		[
                                		{\eg~\citet{cotra2021why, perez2022discovering, wei2023simple, sharma2023towards}}
                                		, cause_leaf, text width=20em
                            		]
                             ]
                        ] 
                    ]
                    [
                        Hallucination from \\ Inference, color=harvestgold!100, fill=harvestgold!60, text=black
                        [
                            Defective Decoding \\ Strategy, color=harvestgold!100, fill=harvestgold!40, text=black
                            [
                            Inherent Sampling \\ Randomness, color=harvestgold!100, fill=harvestgold!20, text=black
                            [
                                {\eg~\citet{stahlberg2019nmt, holtzman2019curious}}
                                , cause_leaf, text width=20em
                            ]
                            ]
                        ]
                        [
                            Imperfect Decoding \\ Representation, color=harvestgold!100, fill=harvestgold!40, text=black
                            [
                            		Insufficient Context \\ Attention, color=harvestgold!100, fill=harvestgold!20, text=black
                            		[
                                		{\eg~\citet{miao2021prevent, chen2022towards, chen2023improving, liu2023instruction}}
                                		, cause_leaf, text width=20em
                            		]
                             ]
                             [
                            		Softmax Bottleneck, color=harvestgold!100, fill=harvestgold!20, text=black
                            		[
                                		{\eg~\citet{yang2017breaking, chang2022softmax}}
                                		, cause_leaf, text width=20em
                            		]
                             ]                        
                         ]
                    ] 
                ]
                [
                    Hallucination \\ Detection and \\ Benchmarks(\S \ref{sec:detection_and_benchmark}), color=cyan!100, fill=cyan!100, text=black
                    [
                        Hallucination Detection, color=cyan!100, fill=cyan!60, text=black
                        [
                            Factuality Hallucination \\ Detection, color=cyan!100, fill=cyan!30, text=black
                            [
                                {\eg~\citet{DBLP:journals/corr/abs-2305-11859, chern2023factool, DBLP:journals/corr/abs-2305-14251}}
                                , detect_leaf, text width=20em
                            ]
                        ]
                        [
                            Faithfulness Hallucination \\ Detection, color=cyan!100, fill=cyan!30, text=black
                            [
                                {\eg~\citet{maynez2020faithfulness, scialom2021questeval, fabbri2021qafacteval}}
                                , detect_leaf, text width=20em
                            ]
                        ]
                    ]
                    [
                        Hallucination Benchmarks, color=cyan!100, fill=cyan!60, text=black
                        [
                            Hallucination Evaluation \\ Benchmarks, color=cyan!100, fill=cyan!30, text=black
                            [
                                {\eg~TruthfulQA \citep{DBLP:conf/acl/LinHE22},HalluQA \citep{cheng2023evaluating}}
                                , detect_leaf, text width=20em
                            ]
                        ]
                        [
                            Hallucination Detection \\ Benchmarks, color=cyan!100, fill=cyan!30, text=black
                            [
                                {\eg~HaluEval\citep{li2023halueval}, FELM\citep{chen2023felm}}
                                , detect_leaf, text width=20em
                            ]
                        ]
                    ]
                ]
                [
                    Hallucination \\ Mitigation (\S \ref{sec:mitigating}), color=lightgreen!100, fill=lightgreen!100, text=black
                    [
                        Mitigating Data-related \\ Hallucinations, color=lightgreen!100, fill=lightgreen!60, text=black
                        [
                            Mitigating Misinformation \\ and Biases, color=lightgreen!100, fill=lightgreen!40, text=black
                            [
                            		Factuality Data \\ Enhancement, color=lightgreen!100, fill=lightgreen!20, text=black
                            		[
                                		{\eg~\citet{gunasekar2023textbooks, touvron2023llama}}
                                , mitigate_leaf, text width=20em
                            		]
                            ]
                            [
                            		Debias, color=lightgreen!100, fill=lightgreen!20, text=black
                            		[
                                		{\eg~\citet{abbas2023semdedup, viswanath2023fairpy, ladhak2023pre}}
                                , mitigate_leaf, text width=20em
                            		]
                            ]
                        ]
                        [
                            Mitigating Knowledge \\ Boundary, color=lightgreen!100, fill=lightgreen!40, text=black
                            [
                            		Model Editing, color=lightgreen!100, fill=lightgreen!20, text=black
                            		[
                                		{\eg~ \citet{mitchell2022memory, huang2023transformer, dai2022neural}}
                                , mitigate_leaf, text width=20em
                            		]
                            ]
                            [
                            		Retrieval Augmentation, color=lightgreen!100, fill=lightgreen!20, text=black
                            		[
                                		{\eg~\citet{DBLP:journals/corr/abs-2302-00083, yu2023improving, DBLP:conf/acl/GaoDPCCFZLLJG23}}
                                , mitigate_leaf, text width=20em
                            		]
                            ]
                        ]
                        [
                            Mitigating Knowledge \\ Shortcut, color=lightgreen!100, fill=lightgreen!40, text=black
                            [
                                Co-occurrence Debias, color=lightgreen!100, fill=lightgreen!20, text=black
                                [
                                		{\eg~\citet{kang2023impact}}
                                , mitigate_leaf, text width=20em
                                ]
                            ]
                        ]
                        [
                            Mitigating Knowledge \\ Recall Failures, color=lightgreen!100, fill=lightgreen!40, text=black
                            [
                                Knowledge Clue \\ Enhancement, color=lightgreen!100, fill=lightgreen!20, text=black
                                [
                                		{\eg~\citet{zheng2023does, wang2023car, tang2023towards}}
                                , mitigate_leaf, text width=20em
                                ]
                            ]
                        ]
                    ]
                    [
                        Mitigating Training-related \\ Hallucinations, color=lightgreen!100, fill=lightgreen!60, text=black
                        [
                            Mitigating Pre-training-\\related Hallucination, color=lightgreen!100, fill=lightgreen!40, text=black
                        [
                            Architecture \\ Improvement, color=lightgreen!100, fill=lightgreen!20, text=black
                            [
                                {\eg~\citet{li2023batgpt, DBLP:journals/corr/abs-2307-03172, liu2023exposing}}
                                , mitigate_leaf, text width=20em
                            ]
                        ]
                        [
                            Pre-training Objective \\ Improvement, color=lightgreen!100, fill=lightgreen!20, text=black
                            [
                                {\eg~\citet{lee2022factuality, shi2023context, wang2023progressive}}
                                , mitigate_leaf, text width=20em
                            ]
                        ]
                        ]
                        [
                            Mitigating Alignment-\\related Hallucination, color=lightgreen!100, fill=lightgreen!40, text=black
                            [
                                Sycophancy, color=lightgreen!100, fill=lightgreen!20, text=black
                            [
                                {\eg~\citet{wei2023simple, sharma2023towards, rimsky2023reducing, rimsky2023modulating}}
                                , mitigate_leaf, text width=20em
                            ]
                            ]
                        ]
                    ]
                    [
                        Mitigating Inference-related \\ Hallucinations, color=lightgreen!100, fill=lightgreen!60, text=black
                        [
                            Factuality Enhanced \\ Decoding, color=lightgreen!100, fill=lightgreen!40, text=black
                        [
                            On Standalone \\ Decoding, color=lightgreen!100, fill=lightgreen!20, text=black
                            [
                                {\eg~\citet{lee2022factuality, li2023inference, chuang2023dola}}
                                , mitigate_leaf, text width=20em
                            ]
                        ]
                        [
                            Post-editing Decoding, color=lightgreen!100, fill=lightgreen!20, text=black
                            [
                                {\eg~\citet{pan2023automatically, dhuliawala2023chain, ji2023towards}}
                                , mitigate_leaf, text width=20em
                            ]
                        ]
                        ]
                        [
                            Faithfulness Enhanced \\ Decoding, color=lightgreen!100, fill=lightgreen!40, text=black
                        [
                            Context Consistency, color=lightgreen!100, fill=lightgreen!20, text=black
                            [
                                {\eg~\citet{wan2023faithfulness, DBLP:journals/corr/abs-2305-14739, DBLP:journals/corr/abs-2306-01286}}
                                , mitigate_leaf, text width=20em
                            ]
                        ]
                        [
                            Logical Consistency, color=lightgreen!100, fill=lightgreen!20, text=black
                            [
                                {\eg~\citet{wang2023scott, o2023contrastive}}
                                , mitigate_leaf, text width=20em
                            ]
                        ]
                        ]
                    ]
            ]
        ]
        ]
        \end{forest}
    }
    \caption{The main content flow and categorization of this survey.}
    \label{categorization_of_survey}
\end{figure*}
